Metropolis-Hastings Data Augmentation for Graph Neural Networks

Graph Neural Networks (GNNs) often suffer from weak-generalization due to sparsely labeled data despite their promising results on various graph-based tasks. Data augmentation is a prevalent remedy to improve the generalization ability of models in many domains. However, due to the non-Euclidean nature of data space and the dependencies between samples, designing effective augmentation on graphs is challenging. In this paper, we propose a novel framework Metropolis-Hastings Data Augmentation (MH-Aug) that draws augmented graphs from an explicit target distribution for semi-supervised learning. MH-Aug produces a sequence of augmented graphs from the target distribution enables flexible control of the strength and diversity of augmentation. Since the direct sampling from the complex target distribution is challenging, we adopt the Metropolis-Hastings algorithm to obtain the augmented samples. We also propose a simple and effective semi-supervised learning strategy with generated samples from MH-Aug. Our extensive experiments demonstrate that MH-Aug can generate a sequence of samples according to the target distribution to significantly improve the performance of GNNs.

==> Sections/4_2.ablation.tex <==

\subsection{Ablation Studies} \label{sec:4.2}

Metropolis-Hastings data augmentation (MH-Aug) and regularizers (Reg) contributes to the entire framework (Table~\ref{table:main}).
As you can see, MH-Aug (w/o Reg) provides considerable gain over all dataset and model. More specifically, it provides 3.25$\%$ performance improvement compared to the vanilla GAT model on Computers. In addition, MH-Aug (w/o Reg) beats DropEdge for all settings and mostly beats AdaEdge which optimizes the graph topology based on the model predictions. 
In the case of CORA (83.55\%) and Computers (80.95\%), it even shows competitive performance over methods leveraging unlabeled data, implying the effectiveness of our sampling-based augmentation itself.
Furthermore, the significant performance gain through regularizer suggests the regularizer we propose is beneficial. In sum, both components contribute to the performance gain.



==> Sections/Preliminaries.tex <==
\section{Preliminaries}
\textbf{Metropolis-Hastings algorithm.} 

\textbf{Ego-graph.}

==> Sections/expression_expansion.tex <==


\begin{align}
\begin{split}
\alpha = &  {p(G^*)q(G|G^*) \over p(G)q(G^*|G)}, \\
p(G) \propto &  \left[ \prod_i \exp{\left( - {(|\Delta G_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 } \right)} \right]^{\lambda_1} \cdot \left[ 1 \over \binom{n}{n\cdot|\Delta G^|} \right]^{\lambda_2} \\
\ln{p(G)} \propto &  \lambda_1 \sum_i{ \left( - {(|\Delta G_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)}
                    - \lambda_2 \ln{\binom{n}{n\cdot|\Delta G|}} \\
q(G|G^*) \propto &  \exp{\left( - {(|\Delta G| - |\Delta G^*|)^2 \over 2{\sigma_\Delta}^2 } \right)} \cdot 
    {1 \over \binom{n}{n\cdot|\Delta x|}}\\
\ln{q(G|G^*)} \propto &  - {(|\Delta G| - |\Delta G^*|)^2 \over 2{\sigma_\Delta}^2 } - \ln{\binom{n}{n\cdot|\Delta x|}}\\
\ln \alpha = & \ln{p(G^*)} - \ln{p(G)} + \ln{q(G|G^*)} - \ln{q(G^*|G)} \\
           = & \quad \lambda_1 \sum_i{ \left( - {(|\Delta G^*_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)}
               - \lambda_2 \ln{\binom{n}{n\cdot|\Delta G^*|}} \\
             & - \lambda_1 \sum_i{ \left( - {(|\Delta G_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)}
               + \lambda_2 \ln{\binom{n}{n\cdot|\Delta G|}} \\
             & - {(|\Delta G| - |\Delta G^*|)^2 \over 2{\sigma_\Delta}^2 } - \ln{\binom{n}{n\cdot|\Delta G|}} \\
             & + {(|\Delta G^*| - |\Delta G|)^2 \over 2{\sigma_\Delta}^2 } - \ln{\binom{n}{n\cdot|\Delta G^*|}} \\
           = & \quad \lambda_1 \sum_i{ \left( - {(|\Delta G^*_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)} - \lambda_1 \sum_i{ \left( - {(|\Delta G_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)} \\
           & + {(|\Delta G^*| - |\Delta G|)^2 \over 2{\sigma_\Delta}^2 } - {(|\Delta G| - |\Delta G^*|)^2 \over 2{\sigma_\Delta}^2 } \\
           &  - (1 - \lambda_2) \ln{\binom{n}{n\cdot|\Delta G|}} + (1 - \lambda_2) \ln{\binom{n}{n\cdot|\Delta G^*|}} \\
           = & \lambda_1 \sum_i{ \left( - {(|\Delta G^*_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)} - \lambda_1 \sum_i{ \left( - {(|\Delta G_i|- \mu )^2 \over 2\sigma(\epsilon_i)^2 }  \right)} \\
           & + {(|\Delta G^*| - |\Delta G|)^2 \over 2{\sigma_\Delta}^2 } - {(|\Delta G| - |\Delta G^*|)^2 \over 2{\sigma_\Delta}^2 } \\
           & - (1 - \lambda_2) \{ \ln{Beta(n - n \cdot |\Delta G| + 1, n \cdot |\Delta G| + 1)} \\
            & \qquad - \ln{Beta(n - n \cdot |\Delta G^*| + 1, n \cdot |\Delta G^*| + 1)} \} \\
, where & \ln{\binom{n}{n\cdot|\Delta G|}} - \ln{\binom{n}{n\cdot|\Delta G^*|}}\\
 = & {n! \over (n - n\cdot|\Delta G^*|)!(n\cdot|\Delta G^*|)!} \cdot {(n - n\cdot|\Delta G^*|)!(n\cdot|\Delta G^*|)! \over  n!} \\
 = & {(n - 1)! \over (n - n\cdot|\Delta G^*|)!(n\cdot|\Delta G^*|)!} \cdot {(n - n\cdot|\Delta G^*|)!(n\cdot|\Delta G^*|)! \over  (n - 1)!} \\
 = & \ln{Beta(n - n \cdot |\Delta G| + 1, n \cdot |\Delta G| + 1)} \\
  & - \ln{Beta(n - n \cdot |\Delta G^*| + 1, n \cdot |\Delta G^*| + 1)}

\end{split} \\
\end{align}


==> Tables/ablation_table2.tex <==
\begin{table}[t] 

  \caption{\textbf{Ablation.} description.} \label{table:ablation}
  \centering
%   \label{ablation2}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{width=1.0\textwidth}    
  \begin{tabular}{cl|ccccc}
    \toprule
    \textbf{BaseGNNs} & \textbf{Method} & \textbf{CORA} & \textbf{CITESEER} & \textbf{Computers} & \textbf{Photo} & \textbf{CS}\\
    \midrule
    \multirow{3}{*}{\textbf{GCN}}
    & Vanilla   & 81.54{\scriptsize$\pm$0.76} & 71.64{\scriptsize$\pm$0.31} & 79.68{\scriptsize$\pm$0.21} & 89.02{\scriptsize$\pm$1.49} & 91.45{\scriptsize$\pm$0.28} \\
 \\
    & +MH-Aug & 83.55{\scriptsize$\pm$0.34} & 72.96{\scriptsize$\pm$0.48} & 80.95{\scriptsize$\pm$2.03} & 89.65{\scriptsize$\pm$1.67} & 91.81{\scriptsize$\pm$0.33} \\

    & +MH-Aug+R & \textbf{85.16{\scriptsize$\pm$0.35}} & \textbf{75.49{\scriptsize$\pm$0.29}} & \textbf{82.80{\scriptsize$\pm$2.08}} & \textbf{90.87{\scriptsize$\pm$1.49}} & \textbf{92.60{\scriptsize$\pm$0.43}} \\
    
    \midrule
    \multirow{3}{*}{\textbf{GraphSAGE}}
    & Vanilla   & 81.54{\scriptsize$\pm$0.76} & 71.64{\scriptsize$\pm$0.31} & 79.68{\scriptsize$\pm$0.21} & 89.02{\scriptsize$\pm$1.49} & 91.45{\scriptsize$\pm$0.28} \\

    & +MH-Aug & 82.46{\scriptsize$\pm$} & 72.12{\scriptsize$\pm$} & 81.74{\scriptsize$\pm$} & 90.37{\scriptsize$\pm$} & 92.24{\scriptsize$\pm$} \\

    & +MH-Aug+R & \textbf{84.70{\scriptsize$\pm$0.39}} & \textbf{75.55{\scriptsize$\pm$0.44}} & \textbf{83.62{\scriptsize$\pm$2.60}} & \textbf{92.19{\scriptsize$\pm$1.37}} & \textbf{93.61{\scriptsize$\pm$0.58}}  \\
    
    \midrule
    \multirow{3}{*}{\textbf{GAT}}
    & Vanilla   & 81.54{\scriptsize$\pm$0.76} & 71.64{\scriptsize$\pm$0.31} & 79.68{\scriptsize$\pm$0.21} & 89.02{\scriptsize$\pm$1.49} & 91.45{\scriptsize$\pm$0.28} \\

    & +MH-Aug & 83.28{\scriptsize$\pm$0.34} & 72.73{\scriptsize$\pm$0.48} & 81.58{\scriptsize$\pm$2.03} & 90.17{\scriptsize$\pm$1.67} & 91.40{\scriptsize$\pm$0.33} \\

    & +MH-Aug+R &  \textbf{84.95{\scriptsize$\pm$0.40}} & \textbf{75.53{\scriptsize$\pm$0.32}} & \textbf{83.25{\scriptsize$\pm$1.88}} & \textbf{90.61{\scriptsize$\pm$1.34}} & \textbf{92.08{\scriptsize$\pm$0.58}} \\
    
    \bottomrule
  \end{tabular}
\end{adjustbox}
\vspace{-5pt}
\end{table} 


==> Tables/algo1.tex <==
\begin{algorithm}
\caption{\label{main} Metropolis-Hastings Data Augmentation (MH-Aug)} 
\textbf{Input:}  $N$\text{ : \#epochs}, $\alpha$, $\beta$, $\theta$
\setstretch{1.3}
\begin{algorithmic}[1]
\State $\G' \leftarrow \G$
\State $\Delta \G' \leftarrow 0$


\For {$n=1$ to $N$}

    \State $\Delta \G^* \sim N(a, b, \Delta \G', \sigma^2_{\Delta})$
    \State $\G^* \leftarrow Drop(\G;\Delta \G^*)$
    \State $u \sim \mathbf{U}(0,1)$
    \If {$u \leq  \min(1, {p(\G^*)q(\G|\G^*) \over p(\G)q(\G^*|\G)})$}

        \State $\mathcal{L}_t \leftarrow
        \mathcal{L}_{s}(\G';\theta) + \lambda_1\mathcal{L}_{u}(\G', \G^*;\theta) + \lambda_2\mathcal{L}_{h}(\G;\theta)$
        
        \State $\text{update } \theta \text{ with } \mathcal{L}_t(\cdot;\theta) $
        \State $\G' \leftarrow \G^*$
        \State $\Delta \G' \leftarrow \Delta \G^*$
        
    \EndIf
\EndFor

\end{algorithmic} 
\end{algorithm}





==> Tables/algo2.tex <==
\begin{algorithm}
\caption{\label{main} MCMC(Markov Chain Monte Carlo)} 
\textbf{Input:}  $N$\text{ : \#epochs}, $\alpha$, $\beta$, $\theta$
\setstretch{1.3}
\begin{algorithmic}[1]
\State $\G' \leftarrow \G$
\State $\Delta \G' \leftarrow 0$


\For {$n=1$ to $N$}

    
    \State $\G^*, \Delta \G^* \leftarrow \text{Aug}(\G,\Delta \G')$
    

    \State $\alpha \leftarrow min(1, {p(\G^*)q(\G|\G^*) \over p(\G)q(\G^*|\G)})$
    \State $u \sim \mathbf{U}(0,1)$
    \If {$u \leq \alpha$}
        \State $\mathcal{L}_t \leftarrow
        \mathcal{L}_{s}(\G';\theta) + \lambda_1\mathcal{L}_{u}(\G', \G^*;\theta) + \lambda_2\mathcal{L}_{h}(\G;\theta)$
        
        \State $\text{update } \theta \text{ with } \mathcal{L}_t(\cdot;\theta) $
        \State $\G' \leftarrow \G^*$
        \State $\Delta \G' \leftarrow \Delta \G^*$
        
    \EndIf
\EndFor

\end{algorithmic} 
\end{algorithm}





==> Tables/data_description_table.tex <==
\begin{table*}[ht] 
    \centering
    \caption{Statistics and details of datasets for node classification.\label{tab:data statistics}}
    \begin{adjustbox}{width=1.0\textwidth}    
    \begin{tabular}{ l  c c c c c c c }
        \toprule
        \multicolumn{1}{ l }{\textbf{Dataset}} & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{\# Features} & \textbf{\# Classes} & \textbf{\# Train} & \textbf{\# Validation} & \textbf{\# Test} \\ \midrule
        \textbf{CORA}               & 2,708   & 5,429     & 1,433  & 7  & 140 & 500  & 1,000 \\ 
        \textbf{CITESEER}           & 3,327   & 4,732      & 3,703  & 6  & 120 & 500  & 1,000 \\ 
        \textbf{Amazon Computers}   & 13,752  & 245,778    & 767   & 10 & 200 & 300  & 13,252 \\ 
        \textbf{Amazon Photo}       & 7,650   & 119,043    & 745   & 8  & 160 & 240 & 7,250 \\
        \textbf{Coauthor CS}        & 18,333  & 81,894    & 6,805  & 15 & 300 & 450  & 17,583 \\
        \textbf{CORA Full}        & 19,793 & 65,311 & 8,710 & 70 & 1,311 & 1,800 & 16,682 \\
        \textbf{ogbn-arxiv}        & 169,343  & 1,166,243    & 128  & 40 & 90,941 & 29,799 & 48,603 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}

\end{table*}

==> Tables/hyperparameter.tex <==
\begin{table}[h] 
  \caption{Hyperparameters of MH-Aug on GCN.} \label{table:table_params}
  \centering
  \label{ablation2}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{width=1.0\textwidth}    
  \begin{tabular}{c|ccccc}
    \toprule
    % \multicolumn{7}{c}{asd}\\
    \textbf{Hyperparameters} & \textbf{CORA} & \textbf{CITESEER} & \textbf{Computers} & \textbf{Photo} & \textbf{CS}\\
    \midrule

    $\alpha_{\E}, \beta_{\E}$ 
    % in linear function of the entropy for edges $\sigma_{\E}(\epsilon_i) = \alpha(\epsilon_i) + \beta$ 
    & 10, 1 & 5, 1 & 10, 1 & 10, 1 & 0, 0.1 \\
    $\alpha_{\V}, \beta_{\V}$ 
    % in linear function of the entropy for nodes $\sigma_{\V}(\epsilon_i) = \alpha(\epsilon_i) + \beta$ 
    & 1, 1 & 10, 0.1 & 10, 0.1 & 10, 1 & 5, 0.1 \\
    % Coefficient of regularizer loss $\mathcal{L}_{u}, 
    $\gamma_1$ & 0.5 & 0.2 & 4 & 3 & 0.2 \\
    % Coefficient of regularizer loss $\mathcal{L}_{h}, 
    $\gamma_2$ & 0.5 & 0.5 & 0.4 & 0.5 & 0.4 \\
    % Standard deviance of proposal distribution for edges and nodes 
    $\sigma_{\Delta,(\E)}$,$\sigma_{\Delta,(\V)}$ & 0.1, 0.01 & 0.005, 0.1 & 0.05, 0.01 & 0.01, 0.005 & 0.001, 0.01 \\ 
    % Mean of target distribution for edges and nodes 
    $\mu_{\E}, \mu_{\V}$ & 0.3, 0.7 & 0.2, 0.5 & 0, 0.1 & 0.5, 0 & 0.8, 0.2 \\ 
    % Influence parameter of distribution with the change ratio of ego-graph $\Delta \G_i$ for edges and nodes, 
    $\lambda_1, \lambda_3$ & 5, 1 & 1, 10  & 1, 10 & 1, 10 & 10, 5 \\
    % Influence parameter of normalization term for edges and nodes, 
    $\lambda_2, \lambda_4$ & 0.9999, 0.999 & 0.9999, 0.999 & 0.9999, 0.9999 & 0.9999, 0.9999 & 0.9999, 1\\
%    num_layers = 2
%    emb_dim = 64
%    dropout = 0.5
    
    \bottomrule
  \end{tabular}
\end{adjustbox}
\label{table:hyperparams}
\vspace{-5pt}
\end{table} 


==> Tables/main_table.tex <==
% \begin{table*}[ht]

% \begin{tabular}{cc|ccccc}
%     \toprule
%     % \multicolumn{2}{c|}{} &
%     % \multicolumn{4}{c}{Dataset} \\
%     %  BaseGNNs & Augmentation & \multicolumn{1}{c}{CORA } & \multicolumn{1}{c}{CITESEER} & \multicolumn{1}{c}{Compu.} & \multicolumn{1}{c}{Photo.}\\
%     \multirow{2}{*}{BaseGNNs} &
%     \multirow{2}{*}{Augmentation}&
%     \multicolumn{4}{c}{Dataset} \\
%     &&
%      \multicolumn{1}{c}{CORA } & \multicolumn{1}{c}{CITESEER} & \multicolumn{1}{c}{Compu.} & \multicolumn{1}{c}{Photo}\\
%     % \midrule
%     % \multirow{1}{*}{MLP} 
%     % & Vanilla   & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33  \\
%     % % \cmidrule{2-7}
%     % & +AugGCR    & \textbf{59.61$\pm$1.53} & \textbf{91.43$\pm$0.72} & \textbf{53.31$\pm$1.95} & \textbf{34.13$\pm$1.04} & \textbf{49.99$\pm$1.60} \\
%     \midrule
%     \multirow{11}{*}{GCN}
%     & Vanilla   & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
%     & DropEdge  & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\  
%     & GAug-O & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GAug-M & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
    
%     & AdaEdge & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & Graph-OVAT & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & UDA(DE) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     % & UDA(DN) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GraphMix & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & SSL & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
    
%     \cmidrule{2-6}
%     & +Ours & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\

%     % & +AugGCR     & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33  \\
    
%     \midrule
%     \multirow{11}{*}{GraphSAGE} 
%     & Vanilla   & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
%     & DropEdge  & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\  
%     & GAug-O & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GAug-M & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
    
%     & AdaEdge & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & Graph-OVAT & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & UDA(DE) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     % & UDA(DN) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GraphMix & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
    
%     \cmidrule{2-6}
%     & +Ours & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\

 
%     \midrule

%     \multirow{11}{*}{GAT} 
%     & Vanilla   & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
%     & DropEdge  & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\  
%     & GAug-O & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GAug-M & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     \cmidrule{2-6}
    
%     & AdaEdge & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & Graph-OVAT & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & UDA(DE) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     % & UDA(DN) & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & GraphMix & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
%     & SSL & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\
    
%     \cmidrule{2-6}
%     & +Ours & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33 & ~53.10$\pm$0.33 \\

%     % & +AugGCR    & ~\textbf{62.57$\pm$0.63} & ~93.26$\pm$0.63 $\downarrow$& ~\textbf{59.55$\pm$1.28} & ~\textbf{28.47$\pm$1.58} & ~\textbf{44.49$\pm$1.61} \\
%     \bottomrule
%   \end{tabular}
% %   \vspace{-0.2cm}
%   \caption{Node classification performance (accuracy) of GNNs trained by various augmentation strategies.} \label{tab:main} % $\downarrow$ indicates the performance degradation by augmentation compared to Vanilla.}  \label{tab:main}

% \end{table*}
\begin{table*}[ht]
% \footnotesize
\caption{Node classification performance (accuracy) of GNNs trained by various methods.} \label{table:main}
\begin{adjustbox}{width=1.0\textwidth}    
\begin{tabular}{cl|ccccc}
    \toprule

    \multirow{2}{*}{\textbf{BaseGNNs}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}}&
    \multicolumn{5}{c}{\textbf{DATASET}} \\
    &&
     \multicolumn{1}{c}{\textbf{CORA} } & \multicolumn{1}{c}{\textbf{CITESEER}} & \multicolumn{1}{c}{\textbf{Compu.}} & \multicolumn{1}{c}{\textbf{Photo}} & \multicolumn{1}{c}{\textbf{CS}}\\

    \midrule
    \multirow{12}{*}{\textbf{GCN}}
    & Vanilla                               & 81.54{\scriptsize$\pm$0.76} & 71.64{\scriptsize$\pm$0.31} & 79.68{\scriptsize$\pm$2.16} & 89.02{\scriptsize$\pm$1.49} & 91.45{\scriptsize$\pm$0.28} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 82.21{\scriptsize$\pm$0.71} & 71.93{\scriptsize$\pm$0.31} & 80.59{\scriptsize$\pm$1.75} & 89.33{\scriptsize$\pm$1.58} & 91.91{\scriptsize$\pm$0.37} \\  
    & GAug-O~\cite{zhao2020data}            & 83.60{\scriptsize$\pm$0.5*} & 73.30*{\scriptsize$\pm$1.1} & OOM & 89.04{\scriptsize$\pm$1.18} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 83.50{\scriptsize$\pm$0.4*} & 72.30{\scriptsize$\pm$0.4*} & 78.90{\scriptsize$\pm$.} & 88.46{\scriptsize$\pm$.} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 83.70{\scriptsize$\pm$1.4*} & 74.10{\scriptsize$\pm$1.4*} & - & - & - \\
    
    \cmidrule{2-7}
    
    & AdaEdge~\cite{chen2020measuring}      & 82.30{\scriptsize$\pm$0.8*} & 69.70{\scriptsize$\pm$0.9*} & 80.66{\scriptsize$\pm$1.227} & 89.94{\scriptsize$\pm$0.84} & 90.30{\scriptsize$\pm$0.4*} \\
    & SSL~\cite{zhu2020self}                & 83.80{\scriptsize$\pm$0.73*} & 72.95{\scriptsize$\pm$0.62*} & - & - & - \\
    & BVAT~\cite{deng2019batch}             & 83.60{\scriptsize$\pm$0.5*} & 74.00{\scriptsize$\pm$0.6*} & 81.20{\scriptsize$\pm$.} & 88.14{\scriptsize$\pm$2.21} & 92.21{\scriptsize$\pm$0.37} \\
    & UDA~\cite{xie2020unsupervised}        & 83.59{\scriptsize$\pm$0.61} & 73.56{\scriptsize$\pm$0.41} & 81.68{\scriptsize$\pm$0.295} & 89.95{\scriptsize$\pm$1.733} & 92.26{\scriptsize$\pm$0.37} \\
    & GraphMix~\cite{verma2019graphmix}     & 83.90{\scriptsize$\pm$0.57*} & 74.70{\scriptsize$\pm$0.59*} & 80.72{\scriptsize$\pm$1.16} & 89.05{\scriptsize$\pm$1.01} & 91.83{\scriptsize$\pm$0.51*} \\
    
    \cmidrule{2-7}
    & +Ours                                 & \textbf{85.16{\scriptsize$\pm$.}} & \textbf{75.49{\scriptsize$\pm$.}} & \textbf{82.80{\scriptsize$\pm$.}} & \textbf{90.81{\scriptsize$\pm$.}} & \textbf{92.56{\scriptsize$\pm$.}} \\

    % & +AugGCR     & ~45.63$\pm$0.64 & ~78.27$\pm$0.29 & ~53.10$\pm$0.33  \\
    
    \midrule
    \multirow{12}{*}{\textbf{GraphSAGE}}
    & Vanilla                               & 79.78{\scriptsize$\pm$0.74} & 71.09{\scriptsize$\pm$0.59} & 79.59{\scriptsize$\pm$0.184} & 89.10{\scriptsize$\pm$1.60} & 91.90{\scriptsize$\pm$0.46} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 80.36{\scriptsize$\pm$0.80} & 71.46{\scriptsize$\pm$0.57} & 79.87{\scriptsize$\pm$1.87} & 89.86{\scriptsize$\pm$1.78} & 92.46{\scriptsize$\pm$0.44} \\  
    & GAug-O~\cite{zhao2020data}            & 82.00{\scriptsize$\pm$0.5*} & 72.70{\scriptsize$\pm$0.7*} & OOM & 88.16{\scriptsize$\pm$2.7} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 83.20{\scriptsize$\pm$0.4*} & 71.20{\scriptsize$\pm$0.4*} & 79.84{\scriptsize$\pm$.} & 88.72{\scriptsize$\pm$.} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 84.10{\scriptsize$\pm$2.4*} & 73.60{\scriptsize$\pm$1.3*} & - & - & - \\
    
    \cmidrule{2-7}
    
    & AdaEdge~\cite{chen2020measuring}      & 80.20{\scriptsize$\pm$1.2*} & 69.40{\scriptsize$\pm$0.8*} & 80.43{\scriptsize$\pm$1.30} & 90.57{\scriptsize$\pm$0.70} & 90.30{\scriptsize$\pm$0.4*} \\
    % & SSL~\cite{zhu2020self} &  &  &  &  &  \\
    & BVAT~\cite{deng2019batch}             & 83.12{\scriptsize$\pm$0.64} & 72.23{\scriptsize$\pm$0.46} & 78.72{\scriptsize$\pm$2.73} & 84.90{\scriptsize$\pm$1.79} & 92.63{\scriptsize$\pm$0.48} \\
    & UDA~\cite{xie2020unsupervised}        & 83.37{\scriptsize$\pm$0.29} & 75.16{\scriptsize$\pm$0.16} & 82.16{\scriptsize$\pm$2.} & 90.61{\scriptsize$\pm$2.} & 92.83{\scriptsize$\pm$0.39} \\
    & GraphMix~\cite{verma2019graphmix}     & 82.28{\scriptsize$\pm$0.55} & 69.62{\scriptsize$\pm$0.36} & 81.33{\scriptsize$\pm$1.46} & 88.46{\scriptsize$\pm$1.36} & 89.29{\scriptsize$\pm$0.45} \\
 
    \cmidrule{2-7}
    & +Ours                                 & \textbf{84.70{\scriptsize$\pm$.}} & \textbf{75.55{\scriptsize$\pm$.}} & \textbf{83.62{\scriptsize$\pm$.}} & \textbf{92.19{\scriptsize$\pm$.}} & \textbf{93.61{\scriptsize$\pm$.}} \\
 
    \midrule

    \multirow{12}{*}{\textbf{GAT}}
    & Vanilla                               & 82.23{\scriptsize$\pm$0.46} & 71.37{\scriptsize$\pm$0.93} & 78.47{\scriptsize$\pm$1.86} & 87.80{\scriptsize$\pm$1.36} & 90.90{\scriptsize$\pm$0.31} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 83.04{\scriptsize$\pm$0.37} & 72.16{\scriptsize$\pm$0.91} & 81.04{\scriptsize$\pm$1.86} & 88.73{\scriptsize$\pm$1.54} & 91.10{\scriptsize$\pm$0.37} \\  
    & GAug-O~\cite{zhao2020data}            & 82.20{\scriptsize$\pm$0.8*} & 71.60{\scriptsize$\pm$1.1*} & OOM & 86.45{\scriptsize$\pm$1.52} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 82.10{\scriptsize$\pm$1.*} & 71.50{\scriptsize$\pm$0.5*} & 77.70{\scriptsize$\pm$.} & 87.08{\scriptsize$\pm$.} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 84.20{\scriptsize$\pm$1.5*} & 73.60{\scriptsize$\pm$2.6*} & - & - & - \\
    
    \cmidrule{2-7}
    
    & AdaEdge~\cite{chen2020measuring}      & 77.90{\scriptsize$\pm$2.0*} & 69.10{\scriptsize$\pm$0.8*} & 77.52{\scriptsize$\pm$1.72} & 88.92{\scriptsize$\pm$0.87} & 86.60{\scriptsize$\pm$0.16*} \\
    & SSL~\cite{zhu2020self}                & 83.70{\scriptsize$\pm$0.61*} & 72.73{\scriptsize$\pm$0.72*} & - & - & - \\
    % & BVAT~\cite{deng2019batch} &  &  &  &  &  \\
    & UDA~\cite{xie2020unsupervised}        & 83.71{\scriptsize$\pm$0.48} & 73.24{\scriptsize$\pm$0.48} & tmp & 89.79{\scriptsize$\pm$1.363} & 91.78{\scriptsize$\pm$0.23} \\
    & GraphMix~\cite{verma2019graphmix}     & 83.32{\scriptsize$\pm$0.18*} & 73.08{\scriptsize$\pm$0.23*} & - & - & - \\
    
    \cmidrule{2-7}
    & +Ours                                 & \textbf{84.81{\scriptsize$\pm$.}} & \textbf{74.59{\scriptsize$\pm$.}} & \textbf{83.13{\scriptsize$\pm$.}} & \textbf{90.53{\scriptsize$\pm$.}} & \textbf{92.08{\scriptsize$\pm$.}} \\

    \bottomrule
  \end{tabular}
  \end{adjustbox}


\end{table*}


==> Tables/table_bak.tex <==

\begin{table*}[ht]
% \footnotesize
\caption{Node classification performance (accuracy) of GNNs trained by various methods.} \label{table:main}
\begin{adjustbox}{width=1.0\textwidth}    
\begin{tabular}{cl|lllll}
    \toprule

    \multirow{2}{*}{\textbf{BaseGNNs}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}}&
    \multicolumn{5}{c}{\textbf{DATASET}} \\
    &&
     \multicolumn{1}{c}{\textbf{CORA} } & \multicolumn{1}{c}{\textbf{CITESEER}} & \multicolumn{1}{c}{\textbf{Compu.}} & \multicolumn{1}{c}{\textbf{Photo}} & \multicolumn{1}{c}{\textbf{CS}}\\
    % \midrule
    \midrule
    \midrule
    
    \multirow{12}{*}{\textbf{GCN}}
    & Vanilla                               & 81.54{\scriptsize$\pm$0.76} & 71.64{\scriptsize$\pm$0.31} & 79.68{\scriptsize$\pm$2.16} & 89.02{\scriptsize$\pm$1.49} & 91.45{\scriptsize$\pm$0.28} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 82.21{\scriptsize$\pm$0.71} & 71.93{\scriptsize$\pm$0.31} & 80.59{\scriptsize$\pm$1.75} & 89.33{\scriptsize$\pm$1.58} & 91.69{\scriptsize$\pm$0.43} \\  
    & GAug-O~\cite{zhao2020data}            & 83.60{\scriptsize$\pm$0.50}$^{\dagger}$ & 73.30{\scriptsize$\pm$1.10}$^{\dagger}$ & OOM & 89.04{\scriptsize$\pm$1.18} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 83.50{\scriptsize$\pm$0.40}$^{\dagger}$ & 72.30{\scriptsize$\pm$0.40}$^{\dagger}$ & 78.90{\scriptsize$\pm$1.76} & 88.46{\scriptsize$\pm$1.24} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 83.70{\scriptsize$\pm$1.40}$^{\dagger}$ & 74.10{\scriptsize$\pm$1.40}$^{\dagger}$ & - & - & - \\
    & AdaEdge~\cite{chen2020measuring}      & 82.30{\scriptsize$\pm$0.80}$^{\dagger}$ & 69.70{\scriptsize$\pm$0.90}$^{\dagger}$ & 80.66{\scriptsize$\pm$1.22} & 89.94{\scriptsize$\pm$0.84} & 90.30{\scriptsize$\pm$0.40}$^{\dagger}$ \\
    
    \cmidrule{2-7}
    
    
    & SSL~\cite{zhu2020self}                & 83.80{\scriptsize$\pm$0.73}$^{\dagger}$ & 72.95{\scriptsize$\pm$0.62}$^{\dagger}$ & - & - & - \\
    & BVAT~\cite{deng2019batch}             & 83.60{\scriptsize$\pm$0.50}$^{\dagger}$ & 74.00{\scriptsize$\pm$0.60}$^{\dagger}$ & 80.07{\scriptsize$\pm$2.41} & 88.46{\scriptsize$\pm$2.25} & 92.21{\scriptsize$\pm$0.37} \\
    & UDA~\cite{xie2020unsupervised}        & 83.59{\scriptsize$\pm$0.61} & 73.56{\scriptsize$\pm$0.41} & 81.68{\scriptsize$\pm$2.95} & 89.95{\scriptsize$\pm$1.73} & 92.26{\scriptsize$\pm$0.37} \\
    & GraphMix~\cite{verma2019graphmix}     & 83.90{\scriptsize$\pm$0.57}$^{\dagger}$ & 74.70{\scriptsize$\pm$0.59}$^{\dagger}$ & 80.72{\scriptsize$\pm$1.16} & 89.05{\scriptsize$\pm$1.01} & 91.83{\scriptsize$\pm$0.51}$^{\dagger}$ \\
    
    \cmidrule{2-7}

    & MH-Aug                                 & \textbf{85.16{\scriptsize$\pm$0.35}} & \textbf{75.49{\scriptsize$\pm$0.29}} & \textbf{82.80{\scriptsize$\pm$2.08}} & \textbf{90.87{\scriptsize$\pm$1.49}} & \textbf{92.60{\scriptsize$\pm$0.43}} \\

    \midrule
    \midrule
    \multirow{12}{*}{\textbf{GraphSAGE}}
    & Vanilla                               & 79.78{\scriptsize$\pm$0.74} & 71.09{\scriptsize$\pm$0.59} & 79.59{\scriptsize$\pm$1.84} & 89.10{\scriptsize$\pm$1.60} & 91.90{\scriptsize$\pm$0.46} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 80.36{\scriptsize$\pm$0.80} & 71.46{\scriptsize$\pm$0.57} & 79.87{\scriptsize$\pm$1.87} & 89.86{\scriptsize$\pm$1.78} & 92.46{\scriptsize$\pm$0.44} \\  
    & GAug-O~\cite{zhao2020data}            & 82.00{\scriptsize$\pm$0.50}$^{\dagger}$ & 72.70{\scriptsize$\pm$0.70}$^{\dagger}$ & OOM & 88.16{\scriptsize$\pm$2.70} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 83.20{\scriptsize$\pm$0.40}$^{\dagger}$ & 71.20{\scriptsize$\pm$0.40}$^{\dagger}$ & 79.84{\scriptsize$\pm$1.99} & 88.72{\scriptsize$\pm$0.97} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 84.10{\scriptsize$\pm$2.40}$^{\dagger}$ & 73.60{\scriptsize$\pm$1.30}$^{\dagger}$ & - & - & - \\
    
    & AdaEdge~\cite{chen2020measuring}      & 80.20{\scriptsize$\pm$1.20}$^{\dagger}$ & 69.40{\scriptsize$\pm$0.80}$^{\dagger}$ & 80.43{\scriptsize$\pm$1.30} & 90.57{\scriptsize$\pm$0.70} & 90.30{\scriptsize$\pm$0.40}$^{\dagger}$ \\
    
    \cmidrule{2-7}

    & BVAT~\cite{deng2019batch}             & 83.12{\scriptsize$\pm$0.64} & 72.23{\scriptsize$\pm$0.46} & 78.72{\scriptsize$\pm$2.73} & 89.40{\scriptsize$\pm$1.79} & 92.63{\scriptsize$\pm$0.48} \\
    & UDA~\cite{xie2020unsupervised}        & 83.37{\scriptsize$\pm$0.29} & 75.16{\scriptsize$\pm$0.16} & 82.16{\scriptsize$\pm$2.00} & 90.61{\scriptsize$\pm$2.00} & 92.83{\scriptsize$\pm$0.39} \\
    & GraphMix~\cite{verma2019graphmix}     & 82.28{\scriptsize$\pm$0.55} & 69.62{\scriptsize$\pm$0.36} & 81.33{\scriptsize$\pm$1.46} & 88.46{\scriptsize$\pm$1.36} & 89.29{\scriptsize$\pm$0.45} \\
 
    \cmidrule{2-7}

    & MH-Aug                                 & \textbf{84.70{\scriptsize$\pm$0.39}} & \textbf{75.55{\scriptsize$\pm$0.44}} & \textbf{83.62{\scriptsize$\pm$2.60}} & \textbf{92.19{\scriptsize$\pm$1.37}} & \textbf{93.61{\scriptsize$\pm$0.58}} \\
 
    \midrule
    \midrule
    \multirow{12}{*}{\textbf{GAT}}
    & Vanilla                               & 82.23{\scriptsize$\pm$0.46} & 71.37{\scriptsize$\pm$0.93} & 78.47{\scriptsize$\pm$1.86} & 87.80{\scriptsize$\pm$1.36} & 90.90{\scriptsize$\pm$0.31} \\
    \cmidrule{2-7}
    & DropEdge~\cite{Rong2020DropEdge:}     & 83.04{\scriptsize$\pm$0.37} & 72.16{\scriptsize$\pm$0.91} & 81.04{\scriptsize$\pm$1.86} & 88.73{\scriptsize$\pm$1.54} & 91.10{\scriptsize$\pm$0.37} \\  
    & GAug-O~\cite{zhao2020data}            & 82.20{\scriptsize$\pm$0.80}$^{\dagger}$ & 71.60{\scriptsize$\pm$1.10}$^{\dagger}$ & OOM & 86.45{\scriptsize$\pm$1.52} & OOM \\
    & GAug-M~\cite{zhao2020data}            & 82.10{\scriptsize$\pm$1.00}$^{\dagger}$ & 71.50{\scriptsize$\pm$0.50}$^{\dagger}$ & 77.70{\scriptsize$\pm$2.10} & 87.08{\scriptsize$\pm$1.00} & OOM \\
    & NeuralSparse~\cite{zheng2020robust}   & 84.20{\scriptsize$\pm$1.50}$^{\dagger}$ & 73.60{\scriptsize$\pm$2.60}$^{\dagger}$ & - & - & - \\
    & AdaEdge~\cite{chen2020measuring}      & 77.90{\scriptsize$\pm$2.00}$^{\dagger}$ & 69.10{\scriptsize$\pm$0.80}$^{\dagger}$ & 77.52{\scriptsize$\pm$1.72} & 88.92{\scriptsize$\pm$0.87} & 86.60{\scriptsize$\pm$0.16}$^{\dagger}$ \\
    
    \cmidrule{2-7}
    
    & SSL~\cite{zhu2020self}                & 83.70{\scriptsize$\pm$0.61}$^{\dagger}$ & 72.73{\scriptsize$\pm$0.72}$^{\dagger}$ & - & - & - \\
    % & BVAT~\cite{deng2019batch} &  &  &  &  &  \\
    & UDA~\cite{xie2020unsupervised}        & 83.71{\scriptsize$\pm$0.48} & 73.24{\scriptsize$\pm$0.48} & 82.42{\scriptsize$\pm$2.95} & 89.79{\scriptsize$\pm$1.36} & 91.78{\scriptsize$\pm$0.23} \\
    & GraphMix~\cite{verma2019graphmix}     & 83.32{\scriptsize$\pm$0.18}$^{\dagger}$ & 73.08{\scriptsize$\pm$0.23}$^{\dagger}$ & - & - & - \\
    
    \cmidrule{2-7}

    & MH-Aug                                 & \textbf{84.95{\scriptsize$\pm$0.40}} & \textbf{75.53{\scriptsize$\pm$0.32}} & \textbf{83.25{\scriptsize$\pm$1.88}} & \textbf{90.61{\scriptsize$\pm$1.34}} & \textbf{92.08{\scriptsize$\pm$0.58}} \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}

\end{table*}

